Rennala NSGD: Asynchronous Stochastic Optimization Beyond Euclidean Geometry

The empirical success of matrix-aware optimizers, such as Muon (Jordan et al., 2024) and Shampoo (arXiv:1802.09568), highlights the potential of non-Euclidean geometry for deep learning, including large language model (LLM) training. Despite this progress, the theoretical understanding of stochastic optimization in general normed spaces remains limited, particularly in distributed settings. We analyze minibatch stochastic gradient descent (SGD) for smooth nonconvex optimization with respect to an arbitrary norm on a finite-dimensional space. Using the framework of $\kappa$-regular normed spaces (arXiv:0809.0813), we derive high-probability oracle complexity bounds under a light-tail condition stated directly in the dual norm induced by the update norm. The bounds make the dependence on geometry explicit through the regularity constant $\kappa$ of the dual space. In the Euclidean case, our bound recovers the standard minibatch SGD rate up to logarithmic factors. For some non-Euclidean geometries and noise models, it is sharper than bounds obtained by converting a Euclidean noise assumption, reducing a linear dimension dependence to a logarithmic one. Building on this framework, we introduce Rennala NSGD, a semi-asynchronous distributed algorithm, and establish wall-clock time complexity guarantees under fixed, heterogeneous worker computation times. In the Euclidean case ($\kappa=1$), our bound matches the parameter dependence of classical Rennala SGD up to logarithmic factors.

==> preamble.tex <==
% !TEX root = arXiv_S_AIRI.tex
\usepackage[utf8]{inputenc} % allow utf-8 input
\usepackage[T1]{fontenc}    % use 8-bit T1 fonts
\usepackage{url}            % simple URL typesetting
\usepackage{booktabs}       % professional-quality tables
\usepackage{amsfonts}       % blackboard math symbols
\usepackage{nicefrac}       % compact symbols for 1/2, etc.
\usepackage{microtype}      % microtypography
%\usepackage[table]{xcolor}         % colors
\usepackage{bbm}
%\usepackage{dsfont}
\usepackage{tcolorbox}
\usepackage{euscript}    %  
\usepackage{makecell}
\usepackage{times}
\RequirePackage{fix-cm}
\usepackage{cmap}                   %   PDF
\usepackage{comment}
\usepackage{xr}
\usepackage{tikz}
%\usepackage{extsizes} %   14- 
\usepackage{csquotes} %   
\usepackage{siunitx}
\usepackage{float}
\restylefloat{table}
%\usepackage{undertilde}
\usepackage{setspace} % 
%\onehalfspacing %  1.5
%\doublespacing %  2
%\singlespacing %  1f
\usepackage[export]{adjustbox}
\usepackage{lastpage} % ,     .
\usepackage{soulutf8} %  
\usepackage{icomma} % "" : $0,2$ --- , $0, 2$ --- 
%\newenvironment{solution}
%{\renewcommand\qedsymbol{$\blacksquare$}\begin{proof}[Solution]}{\end{proof}}
\usepackage{diagbox, eqparbox, hhline}
\usepackage{etoolbox}
\usepackage{mathtools}
\usepackage{etextools}
\usepackage{ifthen}
\usepackage{caption}
\usepackage{subcaption}
\usepackage{amsmath,amssymb, amsthm}
%\usepackage{charter}
%\usepackage{calc}
\usepackage[flushleft]{threeparttable} % http://ctan.org/pkg/threeparttable
\usepackage{calligra}
\usepackage{layout}
\usepackage{lipsum}
%\mathtoolsset{showonlyrefs=true}
\usepackage{mathrsfs}
\usepackage{color}
\usepackage{setspace}
\usepackage{multicol} %  
\usepackage{filecontents}
%nwork with tables
\usepackage{array,tabularx,tabulary,booktabs} %    
\usepackage{colortbl}
%\usepackage{longtable}  %  
\usepackage{multirow} %    
\usepackage{graphicx}
%\usepackage{subfig}
\usepackage{fancyhdr}
\usepackage{theoremref}
\usepackage{pifont}%for defining \xmark
%\usepackage[noend]{algpseudocode}
%\usepackage{verbatim}
%\usepackage[ruled,vlined]{algorithm2e}

\usepackage{algorithm}
% The ICML style used to load `algorithmic` for us; neurips_2026 does not, so
% load it explicitly here (the body uses \STATE/\FOR/\WHILE/... from algorithmic).
\makeatletter
\@ifpackageloaded{algorithmic}{}{\usepackage{algorithmic}}
\makeatother

\usepackage[colorinlistoftodos,bordercolor=orange,backgroundcolor=orange!20,linecolor=orange,textsize=scriptsize]{todonotes}
\usepackage{scalefnt}
\usepackage{xspace}

\makeatletter
\@ifpackageloaded{natbib}{}{\usepackage{natbib}}
\makeatother
\usepackage{hyperref}       % hyperlinks
\usepackage{cleveref}

\usepackage{enumitem}


\usepackage{wrapfig}
\usepackage{listings}
\usepackage{xcolor}
\lstdefinestyle{mystyle}{
    language=Python,
    basicstyle=\ttfamily\small,
    keywordstyle=\color{blue},
    stringstyle=\color{red},
    commentstyle=\color{gray},
    numbers=left,
    numberstyle=\tiny,
    stepnumber=1,
    breaklines=true,
    tabsize=4
}

\usepackage{thmtools}
\usepackage{thm-restate}



\lstset{style=mystyle}


%%%%%%%%%%%%%%
%NEW COMMANDS   %%%
%%%%%%%%%%%%%%
\DeclareMathOperator*{\prox}{prox}
\DeclareMathOperator*{\brox}{brox}


\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}
\DeclareMathOperator*{\minimize}{minimize}
\DeclareMathOperator*{\sign}{sign}
\DeclareMathOperator*{\sgn}{sgn}
\DeclarePairedDelimiter\abs{\lvert}{\rvert}

\newcommand{\z}{\zeta}

\newcommand{\etaj}{\eta_j}
\newcommand{\etajk}{\eta_j^k}

\newcommand{\lt}{\left}
\newcommand{\rt}{\right}
\newcommand{\al}{\alpha}
\newcommand{\p}{\partial}
\newcommand{\oma}{\omega_{\mathrm{av}}}
\newcommand{\Rop}{\mathcal{R}}
\newcommand{\Sop}{\mathcal{S}}
\newcommand{\vv}{v}
\newcommand{\mrate}{c}

\newcommand{\D}{\Delta}
\newcommand{\nfr}{\nicefrac}
\newcommand{\fr}{\frac}
\newcommand{\dfr}{\dfrac}
\newcommand{\mbf}{\mathbf}
\newcommand{\mds}{\mathds}
\newcommand{\bb}{\mathbb}
\newcommand{\wtd}{\widetilde}
\newcommand{\what}{\widehat}
\newcommand{\avg}{\overline}
\newcommand{\wtc}{{\wtd c}}
\newcommand{\wS}{\wtd{S}}
\newcommand{\wA}{\wtd{A}}
\newcommand{\tA}{\tilde{A}}
% \sigmastar macro removed: author uses plain \sigma for the bounded-variance scale (decided 2026-07-05).
\newcommand{\sigmastareff}{\sigma_{*, \mathrm{eff}}}

\newcommand{\sigmt}{\sigma^{t}}
\newcommand{\sigmtpo}{\sigma^{t+1}}
\newcommand{\tB}{\tilde{B}}
\newcommand{\tC}{\tilde{C}}
\newcommand{\ttheta}{\tilde{\theta}}
\newcommand{\inner}[2]{\left\langle #1, #2 \right\rangle}


% \newcommand{\wAi}{\wtd{A}_i}
% \newcommand{\wL}{\wtd{L}}
% \newcommand{\wai}{\wtd{a}_i}
% \newcommand{\wa}{\wtd{a}}
% \newcommand{\wc}{\wtd{c}}

% \newcommand{\wsigma}{\wt{\sigma}}
% \newcommand{\wLi}{\wt{L}_i}
% \newcommand{\wwL}{\wt{\wt{L}}}
% \newcommand{\wB}{\wt{B}}
% \newcommand{\wC}{\wt{C}}
% \newcommand{\ws}{\wt{s}}
% \newcommand{\wg}{\wt{g}}
% \newcommand{\wgt}{\wt{g}^t}
% \newcommand{\wgtpo}{\wt{g}^{t+1}}
% \newcommand{\wht}{\wt{h}^t}
% \newcommand{\whtpo}{\wt{h}^{t+1}}

\newcommand{\wgit}{\wg_i^t}
\newcommand{\wgitpo}{\wg_i^{t+1}}
\newcommand{\wgix}{\wg_i(x)}
\newcommand{\wgiy}{\wg_i(y)}
\newcommand{\wgik}{\wg_i(x^k)}
\newcommand{\wgikpo}{\wg_i(x^{k+1})}

% \newcommand{\wgu}{\wt{g}^u}
% \newcommand{\wG}{\wt{G}}

\newcommand{\hL}{\hat{L}}
\newcommand{\hG}{\hat{G}}
\newcommand{\hAi}{\hat{A}_i}

\newcommand{\hA}{\hat{A}}
\newcommand{\hB}{\hat{B}}
\newcommand{\hC}{\hat{C}}
\newcommand{\hD}{\hat{D}}
\newcommand{\pA}{A^{\prime}}
\newcommand{\pB}{B^{\prime}}
\newcommand{\pC}{C^{\prime}}
\newcommand{\wpA}{\wA^{\prime}}
\newcommand{\wpB}{\wB^{\prime}}
\newcommand{\wpC}{\wC^{\prime}}
\newcommand{\ppA}{A^{\prime \prime}}
\newcommand{\ppB}{B^{\prime \prime}}
\newcommand{\ppC}{C^{\prime \prime}}


\newcommand{\hg}{\hat{g}}
\newcommand{\hatf}{\hat{f}}
\newcommand{\hgi}{\hat{g}_i}
\newcommand{\hgix}{\hat{g}_i(x)}
\newcommand{\hgiy}{\hat{g}_i(y)}
\newcommand{\hgik}{\hat{g}_i(x^k)}
\newcommand{\hgikpo}{\hat{g}_i(x^{k+1})}
\newcommand{\hgit}{\hat{g}_i(x^t)}
\newcommand{\hgitpo}{\hat{g}_i(x^{t+1})}
\newcommand{\hgu}{\hat{g}^u}
\newcommand{\hs}{\hat{s}}


\newcommand{\eik}{e_i^t}
\newcommand{\gik}{g_i^t}
\newcommand{\gikpo}{g_i^{t+1}}
\newcommand{\eikpo}{e_i^{t+1}}
\newcommand{\vik}{v_i^t}
\newcommand{\vikpo}{v_i^{t+1}}

\newcommand{\eit}{e_i^t}
\newcommand{\eitpo}{e_i^{t+1}}
%\newcommand{\vit}{v_i^t}
%\newcommand{\vitpo}{v_i^{t+1}}

% \newcommand{\wcC}{\wt{\cC}}
\newcommand{\La}{\Lambda}
\newcommand{\lam}{\lambda}
\newcommand{\lamt}{\lambda_t}
\newcommand{\lamtpo}{\lambda_{t+1}}
\newcommand{\nut}{\nu_t}
\newcommand{\nutpo}{\nu_{t+1}}
\newcommand{\lami}{\lam_i}
\newcommand{\opn}{\operatorname}
\newcommand{\op}{\operatorname{op}}
\newcommand{\nuc}{\operatorname{nuc}}
\newcommand{\orth}{\operatorname{orth}}


\newcommand{\vp}{\varphi}
\newcommand{\bM}{\mbf M}
\newcommand{\bS}{\mbf S}
\newcommand{\bQ}{\mbf Q}
\newcommand{\bG}{\mbf G}
\newcommand{\bI}{\mbf I}
\newcommand{\bH}{\mbf H}
\newcommand{\bD}{\mbf D}
\newcommand{\bA}{\mbf A}
\newcommand{\bC}{\mbf C}
\newcommand{\bP}{\mbf P}
\newcommand{\bB}{\mbf B}
\newcommand{\bT}{\mbf T}
\newcommand{\bW}{\mbf W}
\newcommand{\bX}{\mbf X}
\newcommand{\bY}{\mbf Y}
\newcommand{\bZ}{\mbf Z}
\newcommand{\bU}{\mbf U}
\newcommand{\bV}{\mbf V}
\newcommand{\bO}{\mbf O}
\newcommand{\bDelta}{{\mbf \Delta}}

\newcommand{\bbB}{\bb B}
\newcommand{\bbU}{\bb U}

\newcommand{\bLa}{\mbf {\La}}
\newcommand{\R}{\bb R}
\newcommand{\bE}{\mbf E}
\newcommand{\hS}{\hat{S}}
\newcommand{\eps}{{\varepsilon}}
\newcommand{\bL}{\mathbf{L}}
\newcommand{\stepsize}{\eta}
\newcommand{\cE}{{\cal E}}
\newcommand{\norm}[1]{\left\| #1 \right\|}
\newcommand{\lin}[1]{\left\langle #1\right\rangle} % product
\newcommand{\linf}[1]{\left\langle #1\right\rangle_{\operatorname{F}}} % product
\newcommand{\cD}{\mathcal{D}}
\newcommand{\cC}{\mathcal{C}}
\newcommand{\cG}{\mathcal{G}}
\newcommand{\cQ}{\mathcal{Q}}
\newcommand{\cK}{\mathcal{K}}
\newcommand{\cF}{\mathcal{F}}
\newcommand{\cL}{\mathcal{L}}
\newcommand{\cI}{\mathcal{I}}

% \newcommand{\wcL}{\wt{\mathcal{L}}}

\newcommand{\cCw}{\cC_{\omega}}
\newcommand{\cCd}{\cC_{\delta}}
\newcommand{\Ctk}[1]{\cC_{Tk}\rb{#1}}
\newcommand{\gixk}{g_{i}(x_k)}
\newcommand{\cS}{\mathcal{S}}
\newcommand{\mM}{\mathbf{M}}
\newcommand{\mN}{\mathbf{N}}
\newcommand{\bN}{\mathbf{N}}
\newcommand{\mI}{\mathbf{I}}
\newcommand{\mL}{\mathbf{L}}
\newcommand{\mD}{\mathbf{D}}
\newcommand{\bx}{\bar{x}}
\newcommand{\by}{\bar{y}}
\newcommand{\barA}{\overline{A}}
\newcommand{\barB}{\overline{B}}
\newcommand{\barL}{\overline{L}}
\newcommand{\barC}{\overline{C}}
\newcommand{\barD}{\overline{D}}
\newcommand{\bara}{\overline{a}}
\newcommand{\eqtext}[1]{\ensuremath{\stackrel{\text{#1}}{=}}}
\newcommand{\letext}[1]{\ensuremath{\stackrel{\text{#1}}{\le}}}
\newcommand{\getext}[1]{\ensuremath{\stackrel{\text{#1}}{\ge}}}
\newcommand{\ltext}[1]{\ensuremath{\stackrel{\text{#1}}{<}}}
\newcommand{\gtext}[1]{\ensuremath{\stackrel{\text{#1}}{>}}}
\newcommand{\succtext}[1]{\ensuremath{\stackrel{\text{#1}}{\succ}}}
\newcommand{\preceqtext}[1]{\ensuremath{\stackrel{\text{#1}}{\preceq}}}

\newcommand{\onenorm}[1]{\left\| #1 \right\|_1}      % norm 
\newcommand{\twonorm}[1]{\left\| #1 \right\|_2}      % norm
\newcommand{\sqtwonorm}[1]{\left\| #1 \right\|^2_2}      % norm
\newcommand{\fnorm}[1]{\left\| #1 \right\|_{\operatorname{F}}}
\newcommand{\sqfnorm}[1]{\left\| #1 \right\|^2_{\operatorname{F}}}
\newcommand{\opf}{\operatorname{F}}


\newcommand{\threenorm}[1]{\left\| #1 \right\|_3}      % norm 
\newcommand{\sqn}[1]{\left\| #1 \right\|^2}
\newcommand{\sqnx}[1]{\left\| #1 \right\|^2_{\boldsymbol{\mathcal{X}}}}
\newcommand{\gnorm}[1]{\left\| #1 \right\|^{1 + \gamma }}      % norm 
\newcommand{\sqnorm}[1]{\left\| #1 \right\|^{2}}
\newcommand{\sqpnorm}[1]{\left\| #1 \right\|^{2}_{+}}
\newcommand{\snorm}[1]{\left\| #1 \right\|_{*}}
\newcommand{\pnorm}[1]{\left\| #1 \right\|_{+}}
\newcommand{\spnorm}[1]{\left\| #1 \right\|_{*,+}}
\newcommand{\sqsnorm}[1]{\left\| #1 \right\|^2_{*}}
\newcommand{\sqspnorm}[1]{\left\| #1 \right\|^2_{*,+}}
\newcommand{\anorm}[1]{\left\| #1 \right\|^{\al}}      % norm 
\newcommand{\bnorm}[1]{\left\| #1 \right\|^{\beta}}      % norm 
\newcommand{\ahnorm}[1]{\left\| #1 \right\|^{\al/2}}      % norm 

\newcommand{\opnorm}[1]{\left\| #1 \right\|_{\op}}      % norm
\newcommand{\infnorm}[1]{\left\| #1 \right\|_{\infty}}      % norm 
\newcommand{\nucnorm}[1]{\left\| #1 \right\|_{\nuc}}      % norm 


\newcommand{\bbone}[1]{\mathbb{1}}      % norm 
\newcommand{\g}{\gamma}
\newcommand{\rbrac}[1]{\left( #1 \right)}


\newcommand{\nf}[1]{\nabla f\rb{#1}}

\newcommand{\whnf}[1]{\widehat{\nabla} f\rb{#1}}

\newcommand{\pf}[1]{\p f\rb{#1}} 
\newcommand{\pfi}[1]{\p f_i\rb{#1}} 

\newcommand{\hotidea}{{\color{red}\bf HOT IDEA: }}
\newcommand{\done}{{\color{blue}\bf DONE: }}
\newcommand{\cO}{{\cal O}}
\newcommand{\cX}{{\cal X}}
\newcommand{\cY}{{\cal Y}}
%\newcommand{\cC}{{\cal C}}
\newcommand{\cT}{{\cal T}}
\newcommand{\cB}{{\cal B}}

\newcommand{\rmX}{{\mathrm X}}
\newcommand{\rmY}{{\mathrm Y}}
\newcommand{\rmZ}{{\mathrm Z}}
\newcommand{\rmF}{{\mathrm F}}

\newcommand{\Dt}{{\Delta}^t}
\newcommand{\Dtpo}{{\Delta}^{t+1}}
\newcommand{\rmXt}{{\mathrm X}^t}
\newcommand{\rmYt}{{\mathrm Y}^t}
\newcommand{\rmZt}{{\mathrm Z}^t}
\newcommand{\rmXtpo}{{\mathrm X}^{t+1}}
\newcommand{\rmYtpo}{{\mathrm Y}^{t+1}}
\newcommand{\rmZtpo}{{\mathrm Z}^{t+1}}



\newcommand{\del}[1]{}

\newcommand{\finf}{f^\mathrm{inf}}
\newcommand{\fiinf}{f_i^\mathrm{inf}}

\let\la=\langle
\let\ra=\rangle


% \def\[{\left[}
%\def\]{\right]}

% \def\({\left(}
% \def\){\right)}
% \def\<{\left\langle}
% \def\>{\right\rangle}


%\newcommand{\st}{\;:\;}
\newcommand{\ve}[2]{\langle #1 ,  #2 \rangle}

%\newcommand{\eqdef}{\stackrel{\text{def}}{=}}
\newcommand{\eqdef}{:=}
\newcommand{\ii}{{}^{(i)}}


\newcommand{\Prob}{\mathbf{Prob}}
\newcommand{\E}{\mathbf{E}}



\newcommand{\vc}[2]{#1^{(#2)}}
\newcommand{\nc}[2]{{\color{red}\|#1\|_{(#2)}}}
\newcommand{\ncs}[2]{\|#1\|^2_{(#2)}}
\newcommand{\ncc}[2]{{\color{red}\|#1\|^*_{(#2)}}}
\newcommand{\ls}[1]{{\color{red} \mathcal S(#1)}}
\newcommand{\Rw}[2]{\mathcal R_{#1}(#2)}
\newcommand{\Rws}[2]{\mathcal R^2_{#1}(#2)}

\newcommand{\nbp}[2]{\|#1\|_{(#2)}}   % norm block primal
\newcommand{\nbd}[2]{\|#1\|_{(#2)}^*} % norm block dual

\newcommand{\lf}{\mathcal L}
\newcommand{\U}{U}
\newcommand{\N}{\bb N}

\newcommand{\mLi}{{\color{red}m^{(i)}}}
\newcommand{\gLi}{{\color{red}f{(i)}}}
%\newcommand{\TLi}{{\color{red}T_L^{(i)}}}
\newcommand{\TLi}[1]{{\color{blue}T^{(#1)}}}

\newcommand{\Lip}{L}

\newcommand{\Rc}[1]{{\color{red}  \mathbf{RC}_{(#1)}}}
\newcommand{\NRCDM}{{\color{red}NRCDM}\  }
\newcommand{\nnz}[1]{{\color{red}\|#1\|_0}}
% sets
\DeclareMathOperator{\card}{card}       % cardinality of a set
\DeclareMathOperator{\diam}{diam}       % diameter of a set
\DeclareMathOperator{\MVEE}{MVEE}       % minim volume enclosing ellipsoid of a set
\DeclareMathOperator{\vol}{vol}         % volume of a set

% statistical
% \DeclareMathOperator{\Exp}{{\rm E}}           % expectation
%\newcommand{\Exp}[1]{{\rm E}\left[#1\right]}
\newcommand{\Exp}[1]{{\bb E}\left[#1\right]}
\newcommand{\Expb}[2]{\mathbb{E}\!\left[\left. #1\,\right|#2 \right]}
\newcommand{\Expc}[1]{\Expb{#1}{\mathcal{F}^t}}
\newcommand{\Expu}[2]{{\bb E}_{#1}\left[#2\right]}
\newcommand{\ExpSub}[2]{{\bb E}_{#1}\left[#2\right]}

\DeclareMathOperator{\Cov}{Cov}         % covariance
\DeclareMathOperator{\Var}{Var}         % variance
\DeclareMathOperator{\Corr}{Corr}       % correlation

% functions and operators
\DeclareMathOperator{\signum}{sign}     % signum/sign of a scalar
\DeclareMathOperator{\dom}{dom}         % domain
\DeclareMathOperator{\epi}{epi}         % epigraph
\DeclareMathOperator{\Ker}{null}        % nullspace/kernel
\DeclareMathOperator{\nullspace}{null}  % nullpsace
\DeclareMathOperator{\range}{range}     % range
\DeclareMathOperator{\Image}{Im}        % image

% topology
\DeclareMathOperator{\interior}{int}    % interior
\DeclareMathOperator{\ri}{rint}         % relative interior
\DeclareMathOperator{\rint}{rint}       % relative interior
\DeclareMathOperator{\bdry}{bdry}       % boundary
\DeclareMathOperator{\cl}{cl}           % closure

% vectors, matrices
\DeclareMathOperator{\linspan}{span}
\DeclareMathOperator{\linspace}{linspace}
\DeclareMathOperator{\cone}{cone}

%\DeclareMathOperator{\tr}{tr}           % trace
\DeclareMathOperator{\rank}{rank}       % rank
\DeclareMathOperator{\conv}{conv}       % convex hull
\DeclareMathOperator{\Diag}{Diag}       % Diag(v) = diagonal matrix with v_i on the diagonal
\DeclareMathOperator{\diag}{diag}       % diag(D) = the diagonal vector of matrix D

\DeclareMathOperator{\Arg}{Arg}         % Argument

%\renewcommand{\qedsymbol}{\ding{114}}

\newcommand{\lamax}[1]{\lam_{\max}\left(#1\right)}
\newcommand{\lamin}[1]{\lam_{\min}\left(#1\right)}
\newcommand{\rb}[1]{\left(#1\right)}
\renewcommand{\sb}[1]{\left[#1\right]}
\newcommand{\cb}[1]{\lt\{#1\rt\}}

\newcommand {\rbl}[1]{(#1)} %round braces without left - right alignment
\renewcommand{\nf}[1]{\nabla f\rbl{#1}}
\newcommand{\nfi}[1]{\nabla f_i\rbl{#1}}
\newcommand{\nfj}[1]{\nabla f_j\rbl{#1}}
\newcommand{\hf}[1]{\nabla^2 f\rbl{#1}}
\newcommand{\hfi}[1]{\nabla^2 f_i\rbl{#1}}

\newcommand{\vtp}{v^{t-1}}
\newcommand{\vt}{v^{t}}
\newcommand{\vtpo}{v^{t+1}}

\newcommand{\yijt}{y_{ij}^t}
\newcommand{\yilt}{y_{il}^t}
\newcommand{\yijtpo}{y_{ij}^{t+1}}
\newcommand{\yiltpo}{y_{il}^{t+1}}
\newcommand{\vitp}{v_i^{t-1}}
\newcommand{\vit}{v_i^{t}}
\newcommand{\vitpo}{v_i^{t+1}}

%\newcommand{\dgit}{\Delta g_i^{t}}
%\newcommand{\dgitpo}{\Delta g_i^{t+1}}
%\newcommand{\dgitpm}{\Delta g_i^{t-1}}
\newcommand{\git}{g_i^t}
\newcommand{\gitpo}{g_i^{t+1}}
\newcommand{\gitpm}{g_i^{t-1}}
\newcommand{\dgit}{\vit}
\newcommand{\dgitpo}{\vitpo}
\newcommand{\dgitpm}{\gitpm}

%\newcommand{\xk}{X^{k}}
\newcommand{\xk}{x^{k}}

\newcommand{\gk}{g^{k}}


\newcommand{\xt}{x^{t}}
\renewcommand{\st}{s^{t}}
\newcommand{\sit}{s_{i}^{t}}
\newcommand{\yt}{y^{t}}
\newcommand{\xtpo}{x^{t+1}}
\newcommand{\ytpo}{y^{t+1}}

\newcommand{\wt}{W^{t}}
\newcommand{\ws}{W^{*}}
\newcommand{\wtpo}{W^{t+1}}
\newcommand{\etpo}{e^{t+1}}


\newcommand{\xitpo}{\xi^{t+1}}
\newcommand{\xit}{\xi^{t}}
\newcommand{\xiit}{\xi_{i}^{t}}

\newcommand{\xijk}{\xi_j^{k}}
\newcommand{\xij}{\xi_{j}}

\newcommand{\xtmo}{x^{t-1}}
\newcommand{\wtdx}{\wtd{x}}
\newcommand{\wtdxk}{\wtd{x}^k}
\newcommand{\wtdxkpo}{\wtd{x}^{k+1}}
% \newcommand{\wtxtpo}{\wt{x}^{t+1}}
% \newcommand{\wtxt}{\wt{x}^{t}}
% \newcommand{\wtgt}{\wt{g}^{t}}

\newcommand{\omtpo}{\omega^{t+1}}
\newcommand{\omt}{\omega^{t}}
\newcommand{\omi}{\omega_i}
\newcommand{\om}{\omega}
% \newcommand{\omi}{w_i}
% \newcommand{\om}{w}

% \newcommand{\omtpo}{w^{t+1}}
% \newcommand{\omt}{w^{t}}

%\newcommand{\xkpo}{X^{k+1}}
\newcommand{\xkpo}{x^{k+1}}

\newcommand{\fxk}{f(\xk)}
\newcommand{\gxk}{g(\xk)}
\newcommand{\fxkpo}{f(\xkpo)}
\newcommand{\dz}{\delta_0}
%\newcommand{\xs}{x^{\star}}
\newcommand{\xs}{x^{*}}
%\newcommand{\xs}{x_{\star}}

\newcommand{\hfxk}{\hf{\xk}}

\newcommand{\nfxk}{\nf{\xk}}
\newcommand{\nfxkpo}{\nf{x^{k+1}}}
\newcommand{\nfxt}{\nf{\xt}}
\newcommand{\nfxtpo}{\nf{\xtpo}}
\newcommand{\nfomt}{\nf{\omt}}
\newcommand{\nfomtpo}{\nf{\omtpo}}
\newcommand{\nfxs}{\nf{\xs}}
\newcommand{\nfx}{\nf{x}}
\newcommand{\nfy}{\nf{y}}
\newcommand{\hfx}{\hf{x}}
\newcommand{\hfy}{\hf{y}}
\newcommand{\nfxijk}{\nabla f_{\xi_{ij}^k} (x^k)}
\newcommand{\nfxijkpo}{\nabla f_{\xi_{ij}^k}(x^{k+1})}
\newcommand{\nfixk}{\nfi{\xk}}
\newcommand{\nfixt}{\nfi{\xt}}
\newcommand{\nfix}{\nfi{x}}
\newcommand{\nfiy}{\nfi{y}}
\newcommand{\nfij}[1]{\nabla f_{ij}\rbl{#1}}
\newcommand{\nfil}[1]{\nabla f_{il}\rbl{#1}}
\newcommand{\nfijxt}{\nfij{\xt}}
\newcommand{\nfijxtpo}{\nfij{\xtpo}}
\newcommand{\nfjxtpo}{\nfj{\xtpo}}
\newcommand{\nfjxt}{\nfj{\xt}}
\newcommand{\nfjomtpo}{\nfj{\omtpo}}
\newcommand{\nfijomiit}{\nfij{\omiit}}
\newcommand{\nfiomiit}{\nfi{\omiit}}
\newcommand{\nfijomiitpo}{\nfij{\omiitpo}}
\newcommand{\nfilomiit}{\nfil{\omiit}}
\newcommand{\nfilomiitpo}{\nfil{\omiitpo}}
\newcommand{\nfilxt}{\nfil{\xt}}
\newcommand{\nfilxtpo}{\nfil{\xtpo}}
\newcommand{\nfijx}{\nabla f_{ij}(x)}
\newcommand{\nfijy}{\nabla f_{ij}(y)}
\newcommand{\dgt}{\Delta g^{t}}
\newcommand{\dgtpo}{\Delta g^{t+1}}
\newcommand{\gt}{ g^{t}}
\newcommand{\gtpo}{ g^{t+1}}

\newcommand{\opern}{\operatorname}
%\newcommand{\omiitpo}{\omega_i^{t+1}}
%\newcommand{\omijt}{\omega_{ij}^{t}}
%\newcommand{\omilt}{\omega_{il}^{t}}
%\newcommand{\omijtpo}{\omega_{ij}^{t+1}}
%\newcommand{\omiltpo}{\omega_{il}^{t+1}}
%\newcommand{\omiit}{\omega_i^{t}}

\newcommand{\omiitpo}{w_i^{t+1}}
\newcommand{\omijt}{w_{ij}^{t}}
\newcommand{\omilt}{w_{il}^{t}}
\newcommand{\omijtpo}{w_{ij}^{t+1}}
\newcommand{\omiltpo}{w_{il}^{t+1}}
\newcommand{\omiit}{w_i^{t}}


\newcommand{\nfiomtpo}{\nfi{\omitpo}}
\newcommand{\nfitpoxtpo}{\nabla f_{i_{t+1}}(x^{t+1})}

%\newcommand{\nfix}{\nfi{x}}

\newcommand{\nfixs}{\nfi{\xs}}
\newcommand{\nfjxk}{\nfj{\xk}}
\newcommand{\nfjxs}{\nfj{\xs}}
\newcommand{\nfixkpo}{\nfi{x^{k+1}}}
\newcommand{\nfixtpo}{\nfi{x^{t+1}}}
\newcommand{\nfitxt}{\nabla f_{i_{t}}(x^{t})}
\newcommand{\nfitomt}{\nabla f_{i_{t}}(\omt)}
%\newcommand{\nfitpoxtpo}{\nabla f_{i_{t+1}}(x^{t+1})}
\newcommand{\nfitpoomtpo}{\nabla f_{i_{t+1}}(\omtpo)}

\newcommand{\nfjxkpo}{\nfj{x^{k+1}}}
\newcommand{\hik}{h^{k}_{i}}
\newcommand{\hikpo}{h^{k+1}_{i}}

\newcommand{\hit}{h^{t}_{i}}
\newcommand{\hitpo}{h^{t+1}_{i}}

%\newcommand{\mit}{m^{t}_{i}}
%\newcommand{\mitpo}{m^{t+1}_{i}}

\newcommand{\ali}{\al_{i}}
\newcommand{\mik}{m^{k}_{i}}
\newcommand{\hk}{h^{k}}
\newcommand{\nmo}{\fr{1}{n}}
\newcommand{\nmt}{\fr{1}{n^2}}
\newcommand{\tnmo}{\fr{2}{n}}
\newcommand{\tnmt}{\fr{2}{n^2}}
\newcommand{\ub}{\underbrace}





\newcommand {\maxin}{\max_{i=1,\dots, n}}
\newcommand {\maxi}{\max_{i}}
\newcommand {\minin}{\min_{i=1,\dots, n}}
\newcommand {\mini}{\min_{i}}
\newcommand {\sumin}{\sum_{i=1}^{n}}
\newcommand {\sumtt}{\sum_{t=0}^{T}}
\newcommand {\sumlmi}{\fr{1}{m_i}\sum_{l=1}^{m_i}}
\newcommand {\suminn}{\fr{1}{n}\sum_{i=1}^{n}}
\newcommand {\sumjm}{\sum_{j=1}^{m}}
\newcommand {\sumjmi}{\sum_{j=1}^{m_i}}
\newcommand {\sumjmm}{\fr{1}{m}\sum_{j=1}^{m}}
\newcommand {\sumim}{\sum_{i=1}^{m}}
\newcommand {\sumimm}{\fr{1}{m}\sum_{i=1}^{m}}
\newcommand {\sumjnn}{\fr{1}{n}\sum_{j=1}^{n}}
\newcommand {\sumjmmi}{\fr{1}{m_i}\sum_{j=1}^{m_i}}
\newcommand {\sumjn}{\sum_{j=1}^{n}}
\newcommand {\sumis}{\sum_{i \in S}}

\newcommand {\wit}{w_{i}^{t}}
\newcommand {\wik}{w_{i}^{k}}
\newcommand {\wjk}{w_{j}^{k}}
\newcommand {\wk}{w^{k}}
\newcommand {\witpo}{w_{i}^{t+1}}
\newcommand {\wikpo}{w_{i}^{k+1}}
\newcommand {\wjkpo}{w_{j}^{k+1}}
%\newcommand {\sumin}{\sum_{i=1}^{n}}
\newcommand {\sumid}{\sum_{i=1}^{d}}
\newcommand {\ghx}{\hat{g}(x)}
\newcommand {\gh}{\hat{g}}
\newcommand {\hx}{\hat{x}}
\newcommand {\gih}{\hat_i}
\newcommand {\gihx}{\hat{g_i}(x)}

%\newcommand {\sumjn}{\sum_{j=1}^{n}}
\newcommand{\cmark}{\textcolor{green}{\ding{51}}}%
\newcommand{\xmark}{\textcolor{red}{\ding{55}}}%

\DeclareMathOperator{\tr}{Tr}

\newcommand{\trace}[1]{\tr\left(#1\right)}
\newcommand{\rbtop}[1]{\left(#1\right)^{\top}}


% \renewcommand{\tr}[1]{\tr\left(#1\right)}






\newtheorem{theorem}{Theorem}
\newtheorem{proposition}{Proposition}

\theoremstyle{plain}

\newtheorem{example}{Example}
\newtheorem{assumption}{Assumption}
\newtheorem{lemma}{Lemma}

\newtheorem{prop}[theorem]{Proposition}
\newtheorem{corollary}{Corollary}
\newtheorem{lem}[theorem]{Lemma}
\newtheorem{claim}[theorem]{Claim}
\newtheorem{remark}{Remark}


\newtheorem{exercise}[theorem]{Exercise}

\newtheorem{rem}[theorem]{Remark}
\newtheorem{que}[theorem]{Question}
\newtheorem{definition}{Definition}


%zerosarah paper symbols

\newcommand*{\qedb}{\hfill\ensuremath{\square}}   % or \blacksquare
\newcommand{\topic}[1]{\vspace{2mm}\noindent{{\bf #1:}}}
\newcommand{\head}[1]{\noindent{{\bf #1:}}}

\definecolor{mylgreen}{rgb}{0.87,1,0.82}
\definecolor{mygreen1}{rgb}{0,0.8,0}
\definecolor{mydarkgreen}{RGB}{39,130,67}
\definecolor{mydarkred}{RGB}{192,47,25}
\definecolor{mydarkblue}{RGB}{39,47,180}
\definecolor{mydarkpurple}{RGB}{48,25,52}
\newcommand\dr[1]{{\color{mydarkred}#1}}
\newcommand\dg[1]{{\color{mydarkgreen}#1}}
\newcommand{\algn}[1]{{\sf\scalefont{0.9}\dr{#1}}\xspace}
\newcommand{\algno}{{\sf\scalefont{0.9}\dr{SILAGE}}\xspace}

\newcommand\gc{\dg{g^*}}
\newcommand\hc{\dr{h^*}}
\newcommand{\green}{\color{mydarkgreen}}
\newcommand{\red}{\color{mydarkred}}
\newcommand{\blue}{\color{mydarkblue}}
\newcommand{\purple}{\color{mydarkpurple}}

\newcommand{\zerosarah}{{\sf ZeroSARAH}\xspace}
\newcommand{\clip}{\operatorname{clip}}
\newcommand{\lmo}{\operatorname*{\mathrm{lmo}}}



\definecolor{lightblue}{RGB}{224, 240, 255} % Adjust RGB values as needed
\definecolor{bgcolor}{rgb}{0.8,1,1}
\definecolor{bgcolor2}{rgb}{0.8,1,0.8}
\newenvironment{proofof}[1]{\smallskip\noindent{\bf \em Proof of #1.}}%





\newcommand{\peter}[1]{\todo[inline]{\textbf{Peter: }#1}}
\newcommand{\igor}[1]{\todo[inline]{\textbf{Igor: }#1}}
\newcommand{\abdurakhmon}[1]{\todo[inline]{\textbf{Abdurakhmon: }#1}}
\newcommand{\hanmin}[1]{\todo[inline]{\textbf{Hanmin: }#1}}

\newcommand{\algname}[1]{{\sf \footnotesize \color{mydarkgreen} #1}\xspace}

\providecommand{\theHalgorithm}{\arabic{algorithm}}


\newcommand{\rA}{{\red A}}
\newcommand{\rB}{{\red B}}
\newcommand{\subgrad}{\tilde{\nabla}}


% \usepackage{titlesec}

% % Define a 4th level heading
% \titleclass{\subsubsubsection}{straight}[\subsubsection]
% \newcounter{subsubsubsection}[subsubsection]
% \renewcommand\thesubsubsubsection{\thesubsubsection.\arabic{subsubsubsection}}

% \titleformat{\subsubsubsection}
%   {\normalfont\normalsize\bfseries}{\thesubsubsubsection}{1em}{}
% \titlespacing*{\subsubsubsection}{0pt}{3.25ex plus 1ex minus .2ex}{1.5ex plus .2ex}

% % Make it numbered and included in the ToC
% \setcounter{secnumdepth}{4}
% \setcounter{tocdepth}{4}

% % Tell LaTeX how to typeset this level inside the .toc
% \makeatletter
% \newcommand*\l@subsubsubsection{\@dottedtocline{4}{10em}{5em}}
% \makeatother

% % (optional) if you use hyperref, also define bookmark level to avoid warnings
% \makeatletter
% \providecommand*{\toclevel@subsubsubsection}{4}
% \makeatother


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Moved here from the main file (arXiv_S_AIRI.tex) to keep the main minimalistic.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\usepackage{empheq}

\newcommand{\squeeze}{\textstyle}
\newcommand{\GD}{\algname{GD}}
\newcommand{\SGD}{\algname{SGD}}
\newcommand{\Muon}{\algname{Muon}}
\newcommand{\AdamW}{\algname{AdamW}}
\newcommand{\DiLoCo}{\algname{DiLoCo}}
\newcommand{\Dion}{\algname{Dion}}

\newtheorem*{example*}{Example}
\newtheorem*{theorem*}{Theorem}

\newtheorem*{exampleone}{Example~\ref{example:1}}
\newtheorem*{exampletwo}{Example~\ref{example:2}}
\newtheorem*{examplethree}{Example~\ref{example:3}}

\newcommand{\intparspace}{\vspace{-0.4em}}
\newcommand{\intsecspace}{\vspace{-0.5em}}

